Light-front holography with chiral symmetry breaking

We present an analytically solvable 3D light-front Hamiltonian model for hadrons that extends light-front holography by including finite mass quarks and a longitudinal confinement term. We propose that the model is suitable as an improved analytic approximation to QCD at a low resolution scale. We demonstrate that it preserves desired Lorentz symmetries and it produces improved agreement with the experimental mass spectroscopy and other properties of the light mesons. Importantly, the model also respects chiral symmetry and the Gell-Mann-Oakes-Renner relation.

==> bibliography.tex <==

\begin{thebibliography}{99}

\bibitem{Vary:2009gt}
J.~P.~Vary, H.~Honkanen, J.~Li, P.~Maris, S.~J.~Brodsky, A.~Harindranath, G.~F.~de Teramond, P.~Sternberg, E.~G.~Ng and C.~Yang,
``Hamiltonian light-front field theory in a basis function approach,''
Phys. Rev. C \textbf{81}, 035205 (2010);
%doi:10.1103/PhysRevC.81.035205
[arXiv:0905.1411 [nucl-th]].


\bibitem{Glazek:2012qj}
S.~D.~Glazek,
``Perturbative formulae for relativistic interactions of effective particles,''
Acta Phys. Polon. B \textbf{43}, 1843-1862 (2012);
%doi:10.5506/APhysPolB.43.1843
[arXiv:1204.4760 [hep-th]].


\bibitem{Glazek:2017rwe}
S.~D.~G\l{}azek, M.~G\'omez-Rocha, J.~More and K.~Serafin,
``Renormalized quark\textendash{}antiquark Hamiltonian induced by a gluon mass ansatz in heavy-flavor QCD,''
Phys. Lett. B \textbf{773}, 172-178 (2017);
%doi:10.1016/j.physletb.2017.08.018
[arXiv:1705.07629 [hep-ph]].

\bibitem{Karch:2006pv}
A.~Karch, E.~Katz, D.~T.~Son and M.~A.~Stephanov,
``Linear confinement and AdS/QCD,''
Phys. Rev. D \textbf{74}, 015005 (2006);
%doi:10.1103/PhysRevD.74.015005
[arXiv:hep-ph/0602229 [hep-ph]].


\bibitem{Brodsky:2013ar}
S.~J.~Brodsky, G.~F.~De T\'eramond and H.~G.~Dosch,
``Threefold Complementary Approach to Holographic QCD,''
Phys. Lett. B \textbf{729}, 3-8 (2014);
%doi:10.1016/j.physletb.2013.12.044
[arXiv:1302.4105 [hep-th]].

\bibitem{deTeramond:2014asa}
G.~F.~de Teramond, H.~G.~Dosch and S.~J.~Brodsky,
``Baryon Spectrum from Superconformal Quantum Mechanics and its Light-Front Holographic Embedding,''
Phys. Rev. D \textbf{91}, no.4, 045040 (2015);
%doi:10.1103/PhysRevD.91.045040
[arXiv:1411.5243 [hep-ph]].

\bibitem{Brodsky:2006uqa}
S.~J.~Brodsky and G.~F.~de Teramond,
``Hadronic spectra and light-front wavefunctions in holographic QCD,''
Phys. Rev. Lett. \textbf{96}, 201601 (2006);
%doi:10.1103/PhysRevLett.96.201601
[arXiv:hep-ph/0602252 [hep-ph]].

\bibitem{Dosch:2016zdv}
H.~G.~Dosch, G.~F.~de Teramond and S.~J.~Brodsky,
``Supersymmetry Across the Light and Heavy-Light Hadronic Spectrum II,''
Phys. Rev. D \textbf{95}, no.3, 034016 (2017);
%doi:10.1103/PhysRevD.95.034016
[arXiv:1612.02370 [hep-ph]].
%38 citations counted in INSPIRE as of 03 Feb 2021

%
\bibitem{Dosch:2015bca}
H.~G.~Dosch, G.~F.~de Teramond and S.~J.~Brodsky,
``Supersymmetry Across the Light and Heavy-Light Hadronic Spectrum,''
Phys. Rev. D \textbf{92}, no.7, 074010 (2015);
%doi:10.1103/PhysRevD.92.074010
[arXiv:1504.05112 [hep-ph]].


\bibitem{Nielsen:2018ytt}
M.~Nielsen, S.~J.~Brodsky, G.~F.~de T\'eramond, H.~G.~Dosch, F.~S.~Navarra and L.~Zou,
``Supersymmetry in the Double-Heavy Hadronic Spectrum,''
Phys. Rev. D \textbf{98}, no.3, 034002 (2018);
%doi:10.1103/PhysRevD.98.034002
[arXiv:1805.11567 [hep-ph]].
%17 citations counted in INSPIRE as of 03 Feb 2021

%\cite{}
\bibitem{Zou:2019tpo}
L.~Zou, H.~G.~Dosch, G.~F.~De T\'eramond and S.~J.~Brodsky,
``Isoscalar mesons and exotic states in light front holographic QCD,''
Phys. Rev. D \textbf{99}, no.11, 114024 (2019);
%doi:10.1103/PhysRevD.99.114024
[arXiv:1901.11205 [hep-ph]].


\bibitem{Brodsky:2008pf}
S.~J.~Brodsky and G.~F.~de Teramond,
``Light-Front Dynamics and AdS/QCD Correspondence: Gravitational Form Factors of Composite Hadrons,''
Phys. Rev. D \textbf{78}, 025032 (2008);
%doi:10.1103/PhysRevD.78.025032
[arXiv:0804.0452 [hep-ph]].

\bibitem{Sufian:2016hwn}
R.~S.~Sufian, G.~F.~de T\'eramond, S.~J.~Brodsky, A.~Deur and H.~G.~Dosch,
``Analysis of nucleon electromagnetic form factors from light-front holographic QCD : The spacelike region,''
Phys. Rev. D \textbf{95}, no.1, 014011 (2017);
%doi:10.1103/PhysRevD.95.014011
[arXiv:1609.06688 [hep-ph]].

\bibitem{deTeramond:2018ecg}
G.~F.~de Teramond \textit{et al.} [HLFHS],
``Universality of Generalized Parton Distributions in Light-Front Holographic QCD,''
Phys. Rev. Lett. \textbf{120}, no.18, 182001 (2018);
%doi:10.1103/PhysRevLett.120.182001
[arXiv:1801.09154 [hep-ph]].
%52 citations counted in INSPIRE as of 05 Feb 2021

\bibitem{Liu:2019vsn}
T.~Liu, R.~S.~Sufian, G.~F.~de T\'eramond, H.~G.~Dosch, S.~J.~Brodsky and A.~Deur,
``Unified Description of Polarized and Unpolarized Quark Distributions in the Proton,''
Phys. Rev. Lett. \textbf{124}, no.8, 082003 (2020);
%doi:10.1103/PhysRevLett.124.082003
[arXiv:1909.13818 [hep-ph]].
%10 citations counted in INSPIRE as of 05 Feb 2021

 \bibitem{Brodsky:2014yha} 
  S.~J.~Brodsky, G.~F.~de Teramond, H.~G.~Dosch and J.~Erlich,
  ``Light-Front Holographic QCD and Emerging Confinement,''
  Phys.\ Rept.\  {\bf 584}, 1 (2015);
%  doi:10.1016/j.physrep.2015.05.001
  [arXiv:1407.8131 [hep-ph]].
  
\bibitem{Brodsky:2020ajy}
S.~J.~Brodsky, G.~F.~de Teramond and H.~G.~Dosch,
``Light-Front Holography and Supersymmetric Conformal Algebra: A Novel Approach to Hadron Spectroscopy, Structure, and Dynamics,''
[arXiv:2004.07756 [hep-ph]].

\bibitem{Gell-Mann:1968}
Murray Gell-Mann, R. J. Oakes, and B. Renner, 
``Behavior of Current Divergences under $SU_3\times SU_3$, 
Phys. Rev. \textbf{175}, 2195 (1968).

\bibitem{Li:2015zda} 
Y.~Li, P.~Maris, X.~Zhao and J.~P.~Vary,
``Heavy Quarkonium in a Holographic Basis,''
Phys.\ Lett.\ B {\bf 758}, 118 (2016);
%  doi:10.1016/j.physletb.2016.04.065
[arXiv:1509.07212 [hep-ph]].
  
  \bibitem{Miller:2019ysh}
G.~A.~Miller and S.~J.~Brodsky,
``Frame-independent spatial coordinate $\tilde{z}$: Implications for light-front wave functions, deep inelastic scattering, light-front holography, and lattice QCD calculations,''
Phys. Rev. C \textbf{102}, no.2, 022201 (2020);
%doi:10.1103/PhysRevC.102.022201
[arXiv:1912.08911 [hep-ph]].

%\cite{Chabysheva:2012fe}
\bibitem{Chabysheva:2012fe}
S.~S.~Chabysheva and J.~R.~Hiller,
``Dynamical model for longitudinal wave functions in light-front holographic QCD,''
Annals Phys. \textbf{337}, 143-152 (2013);
%doi:10.1016/j.aop.2013.06.016
[arXiv:1207.7128 [hep-ph]].
%27 citations counted in INSPIRE as of 21 Feb 2021

%\cite{tHooft:1974pnl}
\bibitem{tHooft:1974pnl}
G.~'t Hooft,
``A Two-Dimensional Model for Mesons,''
Nucl. Phys. B \textbf{75}, 461-470 (1974).
%doi:10.1016/0550-3213(74)90088-1
%1917 citations counted in INSPIRE as of 21 Feb 2021

%\cite{Burkardt:1997de}
\bibitem{Burkardt:1997de}
M.~Burkardt,
``Mesons in a collinear QCD model,''
Phys. Rev. D \textbf{56}, 7105-7118 (1997);
%doi:10.1103/PhysRevD.56.7105
[arXiv:hep-ph/9705224 [hep-ph]].
%12 citations counted in INSPIRE as of 09 Mar 2021

%\cite{Brodsky:2006ez}
\bibitem{Brodsky:2006ez}
S.~J.~Brodsky, S.~Gardner and D.~S.~Hwang,
``Discrete symmetries on the light front and a general relation connecting nucleon electric dipole and anomalous magnetic moments,''
Phys. Rev. D \textbf{73}, 036007 (2006);
%doi:10.1103/PhysRevD.73.036007
[arXiv:hep-ph/0601037 [hep-ph]].
%29 citations counted in INSPIRE as of 11 Feb 2021

\bibitem{rpp:2019}
M. Tanabashi et al. (Particle Data Group), 
``2019 Review of Particle Physics''
Phys. Rev. D 98, 030001 (2018) and 2019 update.

%\cite{Weinberg:1977hb}
\bibitem{Weinberg:1977hb}
S.~Weinberg,
``The Problem of Mass,''
Trans. New York Acad. Sci. \textbf{38}, 185-201 (1977);
%doi:10.1111/j.2164-0947.1977.tb02958.x
%396 citations counted in INSPIRE as of 21 Feb 2021

%\cite{McNeile:2012xh}
\bibitem{McNeile:2012xh}
C.~McNeile, A.~Bazavov, C.~T.~H.~Davies, R.~J.~Dowdall, K.~Hornbostel, G.~P.~Lepage and H.~D.~Trottier,
``Direct determination of the strange and light quark condensates from full lattice QCD,''
Phys. Rev. D \textbf{87}, no.3, 034503 (2013);
%doi:10.1103/PhysRevD.87.034503
[arXiv:1211.6577 [hep-lat]].
%94 citations counted in INSPIRE as of 09 Mar 2021

\bibitem{pdg:2020}
P.A. Zyla et al. (Particle Data Group), Prog. Theor. Exp. Phys. 2020, \textbf{083C0}1 (2020).

  \bibitem{Gutsche:2012ez} 
  T.~Gutsche, V.~E.~Lyubovitskij, I.~Schmidt and A.~Vega,
  ``Chiral Symmetry Breaking and Meson Wave Functions in Soft-Wall AdS/QCD,''
  Phys.\ Rev.\ D {\bf 87}, no. 5, 056001 (2013);
%  doi:10.1103/PhysRevD.87.056001
  [arXiv:1212.5196 [hep-ph]].

\bibitem{Tang:2018myz}
S.~Tang, Y.~Li, P.~Maris and J.~P.~Vary,
``$B_c$ mesons and their properties on the light front'',
Phys. Rev. D \textbf{98}, no.11, 114038 (2018);
%doi:10.1103/PhysRevD.98.114038
[arXiv:1810.05971 [nucl-th]].
%21 citations counted in INSPIRE as of 25 Oct 2020

%\cite{Tang:2019gvn}
\bibitem{Tang:2019gvn}
S.~Tang, Y.~Li, P.~Maris and J.~P.~Vary,
``Heavy-light mesons on the light front'',
Eur. Phys. J. C \textbf{80}, no.6, 522 (2020);
%doi:10.1140/epjc/s10052-020-8081-9
[arXiv:1912.02088 [nucl-th]].

\bibitem{Qian:2020utg}
W.~Qian, S.~Jia, Y.~Li and J.~P.~Vary,
``Light mesons within the basis light-front quantization framework,''
Phys. Rev. C \textbf{102}, no.5, 055207 (2020);
%doi:10.1103/PhysRevC.102.055207
[arXiv:2005.13806 [nucl-th]].

%\cite{Jia:2018ary}
\bibitem{Jia:2018ary}
S.~Jia and J.~P.~Vary,
``Basis light front quantization for the charged light mesons with color singlet Nambu\textendash{}Jona-Lasinio interactions,''
Phys. Rev. C \textbf{99}, no.3, 035206 (2019);
%doi:10.1103/PhysRevC.99.035206
[arXiv:1811.08512 [nucl-th]].
%26 citations counted in INSPIRE as of 24 Feb 2021

%\cite{Brodsky:2010xf}
\bibitem{Brodsky:2010xf}
S.~J.~Brodsky, C.~D.~Roberts, R.~Shrock and P.~C.~Tandy,
``Essence of the vacuum quark condensate,''
Phys. Rev. C \textbf{82}, 022201 (2010);
%doi:10.1103/PhysRevC.82.022201
[arXiv:1005.4610 [nucl-th]].
%130 citations counted in INSPIRE as of 09 Mar 2021

\bibitem{Li:2017mlw}
Y.~Li, P.~Maris and J.~P.~Vary,
``Quarkonium as a relativistic bound state on the light front,''
Phys. Rev. D \textbf{96}, no.1, 016022 (2017);
%doi:10.1103/PhysRevD.96.016022
[arXiv:1704.06968 [hep-ph]].

%\bibitem{Glazek:2017rwe}
%S.~D.~G\l{}azek, M.~G\'omez-Rocha, J.~More and K.~Serafin,
%``Renormalized quark\textendash{}antiquark Hamiltonian induced by a gluon mass ansatz in heavy-flavor QCD,''
%Phys. Lett. B \textbf{773}, 172-178 (2017);
%%doi:10.1016/j.physletb.2017.08.018
%[arXiv:1705.07629 [hep-ph]].

\end{thebibliography}
